Evaluation of autonomous systems under data distribution shifts

We posit that data can only be safe to use up to a certain threshold of the data distribution shift, after which control must be relinquished by the autonomous system and operation halted or handed to a human operator. With the use of a computer vision toy example we demonstrate that network predictive accuracy is impacted by data distribution shifts and propose distance metrics between training and testing data to define safe operation limits within said shifts. We conclude that beyond an empirically obtained threshold of the data distribution shift, it is unreasonable to expect network predictive accuracy not to degrade

==> cvpr2023/latex/sections/06-Leftovers.tex <==
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of cvpr.sty to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the CVPR70 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.


% Update the cvpr.cls to do the following automatically.
% For this citation style, keep multiple citations in numerical (not
% chronological) order, so prefer \cite{Alpher03,Alpher02,Authors14} to
% \cite{Alpher02,Alpher03,Authors14}.


\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

%------------------------------------------------------------------------
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

%------------------------------------------------------------------------
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% EXPERIMENTS

We examined the same scenario in YUV space, first we generated the corresponding plot to Figure \ref{fig:HI_KL_DB_safe}. By comparing one image to the shifted versions of the same image, with shifts ranging from negative to positive 120, totalling 241 and including a "zero" shift which is comparing the image to the same image with no shift, generating the maximum value of 1 for the Histogram Intersection and zero for both Relative Entropy and Bhattacharyya Distance.

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{Images/HI_KL_DB_YUV_safe.png}
\caption{Histogram Intersection, Relative Entropy and Bhattacharyya Distance safe limits for YUV image pixel intensity value shifts}
\label{fig:HI_KL_DB_YUV_safe}
\end{figure}

\begin{table}[ht!]
\caption{Histogram Intersection in YUV space between random Generated Road frames}
\label{table:histogram_intersection_yuv_space}
\begin{center}
\begin{tabular}{llllllllll}
\toprule
& ID1 & ID2 & -120 & -80 & -40 & 0 & 40 & 80 & 120 \\
\midrule
1 & 592 & 503 & 0.02 & \textbf{0.06} & 0.09 & 0.71 & 0.16 & \textbf{0.06} & 0.02 \\
2 & 863 & 825 & 0.02 & 0.02 & 0.14 & 0.69 & 0.07 & 0.02 & 0.01 \\
3 & 912 & 879 & 0.02 & 0.04 & 0.11 & 0.72 & 0.03 & 0.02 & 0.01 \\
4 & 1096 & 410 & 0.01 & 0.04 & 0.17 & 0.57 & 0.03 & 0.02 & 0.01 \\
5 & 519 & 772 & 0.03 & 0.06 & 0.18 & 0.61 & 0.09 & 0.03 & 0.02 \\
6 & 365 & 1091 & 0.02 & 0.03 & 0.05 & 0.61 & 0.18 & 0.04 & 0.01 \\
7 & 1082 & 1094 & 0.01 & 0.01 & 0.03 & 0.82 & 0.03 & 0.02 & 0.01 \\
8 & 811 & 1300 & 0.01 & 0.02 & \textbf{0.03} & \textbf{0.50} & \textbf{0.21} & 0.04 & 0.01 \\
9 & 146 & 1004 & 0.01 & 0.02 & 0.05 & 0.80 & 0.06 & 0.03 & 0.02 \\
10 & 1199 & 593 & 0.02 & 0.05 & 0.19 & 0.59 & 0.08 & 0.04 & 0.02 \\
11 & 797 & 1157 & 0.01 & 0.02 & \textbf{0.03} & \textbf{0.50} & \textbf{0.20} & 0.04 & 0.01 \\
12 & 350 & 173 & 0.01 & 0.02 & 0.05 & 0.56 & 0.18 & 0.05 & 0.01 \\
13 & 407 & 1260 & 0.01 & 0.02 & 0.03 & 0.56 & 0.18 & 0.05 & 0.02 \\
14 & 157 & 1036 & 0.01 & 0.02 & 0.04 & 0.78 & 0.03 & 0.02 & 0.00 \\
15 & 331 & 1139 & 0.02 & 0.03 & 0.06 & 0.64 & 0.18 & 0.04 & 0.01 \\
16 & 623 & 1259 & 0.01 & 0.03 & 0.07 & 0.62 & 0.16 & 0.05 & 0.02 \\
17 & 235 & 566 & 0.01 & 0.02 & 0.16 & 0.72 & 0.14 & 0.04 & 0.01 \\
18 & 950 & 458 & 0.02 & 0.04 & 0.22 & 0.62 & 0.03 & 0.02 & 0.01 \\
19 & 1237 & 158 & 0.01 & 0.02 & 0.04 & 0.78 & 0.04 & 0.02 & 0.01 \\
20 & 850 & 1011 & 0.01 & 0.02 & 0.03 & 0.67 & 0.11 & 0.05 & 0.03 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

In YUV space we notice that the plot in Figure \ref{fig:HI_KL_DB_YUV_safe}, as mentioned previously, is more exponential than linear. For the Histogram Intersection distance metric we notice that for shift less than negative 40 or greater than negative 40 there is no more information given as the metric is close to zero, than is, any change of more than or less than 40 pixels, implies there is no histogram overlap and the images may have been arbitrarily shifted into a space that cannot be quantified as well as had it been in RGB space. If we were to use the same reasoning with respect to YUV space, and claim that we would need a Histogram Intersection of no less than 0.10 to accept the network prediction as safe to use, we look at columns negative and positive 40 and see that we are discarding a majority of predictions. We look at the projection onto the x axis, given a y axis value of 0.10 for the Histogram Intersection, and determine that the limits are closer to negative and positive 30. We discard the Histogram Intersection in YUV space as a distance metric, as it cannot represent enough distance information.

\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{Images/Frames_100_1300_HI_KL_DB_safe.png}
\caption{Histogram Intersection, Relative Entropy and Bhattacharyya Distance in RGB space between frame 100 and others up to frame 1300, with safe limit}
\label{fig:Frames_100_1300_HI_KL_DB_safe}
\end{figure}

\newpage
\begin{table}[ht!]
\caption{Relative Entropy in YUV space between random Generated Road frames}
\label{table:relative_entropy_yuv_space}
\begin{center}
\begin{tabular}{llllllllll}
\toprule
& ID1 & ID2 & -120 & -80 & -40 & 0 & 40 & 80 & 120 \\
\midrule
1 & 592 & 503 & 2.72 & 2.50 & 2.35 & 0.14 & 2.24 & 2.48 & 2.73 \\
2 & 863 & 825 & 2.88 & 2.72 & 2.33 & 0.17 & 2.76 & 2.89 & 2.92 \\
3 & 912 & 879 & 2.68 & 2.54 & 2.33 & 0.16 & 2.76 & 2.84 & 2.86 \\
4 & 1096 & 410 & 2.80 & 2.63 & 2.28 & 0.30 & 2.65 & 2.94 & 2.96 \\
5 & 519 & 772 & 2.76 & \textbf{2.48} & 2.29 & 0.21 & 2.37 & 2.67 & 2.80 \\
6 & 365 & 1091 & 2.65 & 2.53 & 2.38 & 0.30 & 2.22 & 2.59 & 2.69 \\
7 & 1082 & 1094 & 2.80 & 2.67 & 2.63 & 0.07 & 2.65 & 2.92 & 2.94 \\
8 & 811 & 1300 & 2.94 & 2.72 & \textbf{2.60} & \textbf{0.42} & \textbf{2.28} & 2.60 & 2.92 \\
9 & 146 & 1004 & 2.67 & 2.54 & 2.45 & 0.08 & 2.39 & 2.79 & 2.81 \\
10 & 1199 & 593 & 2.63 & 2.50 & 2.14 & 0.32 & 2.31 & 2.72 & 2.79 \\
11 & 797 & 1157 & 2.88 & 2.69 & 2.55 & 0.41 & 1.98 & 2.69 & 2.87 \\
12 & 350 & 173 & 2.72 & 2.64 & 2.44 & 0.40 & 2.25 & 2.61 & 2.72 \\
13 & 407 & 1260 & 2.83 & 2.67 & 2.52 & 0.31 & \textbf{1.97} & 2.53 & 2.77 \\
14 & 157 & 1036 & 2.81 & 2.62 & 2.61 & 0.09 & 2.74 & 2.93 & 2.95 \\
15 & 331 & 1139 & 2.72 & 2.57 & 2.42 & 0.27 & 2.23 & 2.60 & 2.73 \\
16 & 623 & 1259 & 2.75 & 2.62 & 2.42 & 0.30 & \textbf{1.97} & 2.57 & 2.75 \\
17 & 235 & 566 & 2.85 & 2.75 & 2.40 & 0.18 & 2.33 & 2.70 & 2.92 \\
18 & 950 & 458 & 2.69 & 2.57 & 2.17 & 0.27 & 2.62 & 2.85 & 2.88 \\
19 & 1237 & 158 & 2.88 & 2.66 & 2.57 & 0.11 & 2.63 & 2.86 & 2.88 \\
20 & 850 & 1011 & 2.97 & 2.73 & 2.68 & 0.22 & 2.46 & 2.67 & 2.87 \\

\bottomrule
\end{tabular}
\end{center}
\end{table}

To visualise the Histogram Intersection, Relative Entropy and Bhattacharyya Distance between one frame and all following frames, we selected frame 100 from the Generated Track and measured the distance between that frame and all following frames up to 1300, plotting the result on Figure \ref{fig:Frames_100_1300_HI_KL_DB_safe}. We choose an arbitrary horizontal "safe" line and observe that the metric furthest from the line is the Bhattacharyya Distance and perhaps in this scenario, the best one to use, as it has the smallest delta between all computed distances, the idea being the prediction can be seen as safe as long as the plot does not cross the line.

Table \ref{table:relative_entropy_yuv_space} shows the Relative Entropy values in YUV space, analogous to Table \ref{table:re_rgb_space} in RGB space. We again highlight the largest value, that is the furthest distance, between images ID1 and ID2. We notice and the shift column in YUV space, less than and include negative 40 and greater and including positive 40 quickly saturate, reflecting the exponential rate at which the distance is changing in YUV space. If a distance of 2 or less is accepted, we are likely in the range of negative to positive 20 as can be inferred in Figure \ref{fig:HI_KL_DB_YUV_safe}. Again the exponential relation between shift and distance determines that, as the value converge asymptotically to the limits, we lose information in the limits and can no longer obtain any useful metrics outside a very narrow range of pixel intensity shifts.

We compare and contrast the RGB and YUV distances between frame 100 and all following frames up to 1300 by plotting Figure \ref{fig:Frames_100_1300_HI_KL_DB_YUV_safe}. We see that the Histogram Intersection values have the highest values near 0.8, compared to near 1 in RGB space, although the delta in YUV space is smaller. We see once again that the Bhattacharyya Distance is the best metric, as it is the furthest from our arbitrarily chosen "safe" cyan horizontal line. We see in Figure \ref{fig:HI_KL_DB_YUV_safe} that the Bhattacharyya Distance, in the negative to positive 50 pixel intensive shift range, is the most linear of the three metrics analysed.


\begin{figure}[h!]
\centering
\includegraphics[width=\textwidth]{Images/Frames_100_1300_HI_KL_DB_YUV_safe.png}
\caption{Histogram Intersection, Relative Entropy and Bhattacharyya Distance in YUV space between frame 100 and others up to frame 1300 with safe limit}
\label{fig:Frames_100_1300_HI_KL_DB_YUV_safe}
\end{figure}


\begin{table}[ht!]
\caption{Bhattacharyya Distance in YUV space between random Generated Road frames}
\label{table:bhattacharyya_distance_yuv}
\begin{center}
\begin{tabular}{llllllllll}
\toprule
& ID1 & ID2 & -120 & -80 & -40 & 0 & 40 & 80 & 120 \\
\midrule
1 & 592 & 503 & 3.51 & 2.14 & 1.62 & 0.07 & 1.41 & \textbf{1.97} & 3.33 \\
2 & 863 & 825 & 3.66 & 2.74 & 1.37 & 0.10 & 2.00 & 2.76 & 4.39 \\
3 & 912 & 879 & 3.02 & 2.35 & 1.45 & 0.08 & 2.39 & 2.72 & 3.83 \\
4 & 1096 & 410 & 3.20 & 2.41 & 1.31 & 0.20 & 2.23 & 2.95 & 4.46 \\
5 & 519 & 772 & 2.90 & \textbf{1.84} & 1.35 & 0.13 & 1.63 & 2.44 & 3.59 \\
6 & 365 & 1091 & 3.56 & 2.74 & 1.73 & 0.16 & 1.37 & 2.34 & 3.29 \\
7 & 1082 & 1094 & 3.44 & 2.85 & 2.32 & 0.03 & 2.33 & 2.80 & 3.45 \\
8 & 811 & 1300 & 4.95 & 2.91 & 2.35 & 0.24 & 1.23 & 2.11 & 3.27 \\
9 & 146 & 1004 & 3.24 & 2.68 & 1.85 & 0.05 & 1.82 & 2.57 & 3.07 \\
10 & 1199 & 593 & 2.87 & 2.07 & 1.25 & 0.18 & 1.67 & 2.50 & 3.43 \\
11 & 797 & 1157 & 4.64 & 2.90 & \textbf{2.22} & \textbf{0.24} & \textbf{1.20} & 2.35 & 3.67 \\
12 & 350 & 173 & 4.12 & 3.16 & 1.85 & 0.20 & 1.38 & 2.29 & 3.32 \\
13 & 407 & 1260 & 4.71 & 3.01 & 2.37 & 0.18 & \textbf{1.20} & 2.01 & 2.87 \\
14 & 157 & 1036 & 3.44 & 2.70 & 2.38 & 0.06 & 2.29 & 2.94 & 3.89 \\
15 & 331 & 1139 & 3.64 & 2.66 & 1.81 & 0.15 & 1.32 & 2.25 & 3.21 \\
16 & 623 & 1259 & 3.73 & 2.78 & 1.72 & 0.18 & 1.28 & 2.16 & 2.98 \\
17 & 235 & 566 & 3.54 & 2.88 & 1.55 & 0.11 & 1.44 & 2.36 & 3.87 \\
18 & 950 & 458 & 2.88 & 2.06 & 1.20 & 0.17 & 2.24 & 2.81 & 4.35 \\
19 & 1237 & 158 & 4.72 & 2.95 & 1.93 & 0.06 & 2.28 & 2.75 & 3.47 \\
20 & 850 & 1011 & 4.45 & 2.78 & 2.30 & 0.13 & 1.50 & 2.02 & 2.71 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}

Table \ref{table:bhattacharyya_distance_yuv} shows the corresponding analysis in YUV space, analogous to Table \ref{table:bhattacharyya_distance_rgb_space}. Row 11 is highlighted to show the highest value (furthest distance) between two randomly chosen images from the Generated Track dataset. We then look at the distances for columns negative and positive 40 shifts on the same row. We then look for the minimum values on columns negative and positive 80, and determine that the minimum acceptable value for the metric, between a randomly chosen training dataset image, and an image acquired by the autonomous system is approximately 1.80 or less. Which is approximately in the negative and positive 35 pixel intensity shift range as shown in Figure \ref{fig:HI_KL_DB_YUV_safe}, and perhaps the only useful data distribution shift metric in YUV space.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CONCLUSIONS

We generated over ten million predictions to gather data for our initial evaluation of autonomous systems under data distribution shifts. We noticed that Histogram Intersection, Relative Entropy and Bhathacharyya Distance carry more information in RGB space given the linear relation between pixel intensity shift and distance metric in RGB space, and a corresponding exponential relation in YUV space. We observed that Histogram Intersection is the preferred choice if RGB space is used, and the Bhattacharyya Distance is the preferred metric if YUV space is used for determining data distribution shift between data used to train the model and real world data. We observed that MAE is the most computationally efficient metric for network accuracy error quantification.

Comparing the RGB space distance plots in Figure \ref{fig:HI_KL_DB_YUV_safe}, with the steering error plots in Figures 
\ref{fig:dataShiftedSteeringPredictions-0m40m80m120},
\ref{fig:dataShiftedSteeringPredictions-p40p80p120},
\ref{fig:nvidia1_dataShiftedSteeringPredictions-0m40m80m120} and
\ref{fig:nvidia1_dataShiftedSteeringPredictions-p40p80p120}, we
could make claims such as, given an autonomous system driven by an ensemble of two models, nvidia1 and nvidia2, where the prediction is an average of both outputs, we would consider the input data safe to use as long as the RGB Histogram Intersection between a randomly chosen image from the training dataset, and an image acquired from the autonomous vehicle's camera, is greater than a given amount, 
or as long as the YUV Bhatthacharya Distance under the same circumstances, was smaller than a given amount. Otherwise the network prediction generated from
the acquired image is not safe to use and the autonomous system control should be deferred to a human operator. 

A formulation could be given by defining a range of maximum and minimum pixels intensity value averages, over the entire training dataset, and the allowed data distribution shift. The output being a boolean value where true means the image and resulting prediction are safe to use, false otherwise.

We first define a safe range:

\begin{equation}
    sr = ((S_{pos}-S_{neg})-(RGB_{max} - RGB_{min}))2^{-1}
\end{equation}

Where $S_{pos, S_{neg}}$ is the safe data shift range observed empirically, and $RGB_{max}, RGB_{min}$ is the expected range of RGB average values. $sr$ therefore is the safe absolute value change, such that the resulting distribution shift would be within the range $S_{pos},S_{neg}$.

\begin{equation}
    P_{safe} = 
    \begin{cases}
    true , & \text{if $|D_Brgb(P,Q)| < |D_Brgb(P,Q_{sr})|$}.\\
    true, & \text{if $|D_\text{KLrgb}(P \parallel Q)| < |D_\text{KLrgb}(P \parallel Q_{sr})|$}.\\
    true, & \text{if $|H_{irgb}(P, Q)| > |H_{irgb}(P, Q_{sr})|$}. \\
    false ,  & \text{otherwise}.
    \end{cases}
\end{equation}
Where $P_{safe}$ is a boolean value determining if it is safe to make a prediction from input $Q$ relative to $Q_{sr}$, and $Q_{sr}$ is a range betwee negative and positive $sr$, and the comparisons are performed in RGB space.
Given the computational advantages, and strong linearity
$H_{irgb}$ is the preferred distance metric. Also, distance metrics are more meaningful in RGB than YUV space, where the functions grow asymptotically faster.
To validate the hypothesis further, simulations would be required to assert $P_{safe}$ holds in the order of hundreds of millions, even billions of miles driven, repeatable for a number of specific scenarios e.g. obstacle avoidance, unexpected noise and lighting conditions and others to be determined.

%We can express our accuracy, given a data shift as:

%%\begin{equation}
 %   A_(D, \delta) = |A(d)-A(\delta)|  
%\end{equation}

%Number of parameters, which can be taken as a proxy for network geometry, can also be a useful measure for accuracy, it could be shown that:

%\begin{equation}
%    A_(D_s) = |A(d)-A(d-\sigma)|
%\end{equation}

%\subsection{Network parameters}
%Here we discuss the topic of overfitting, number of parameters in the CNN and our objective of comparing number of parameters, accuracy and accuracy change as a function of data distribution shift such as:

%$
%A_C(D_s) = |A(d)-A(d-\sigma)|
%$

%we want to be able to claim that 1. an optimal number of parameters, What is the optimal number of parameters? We could overparametirize and overfit as is often the case \cite{bengios_brother}. We could underparameterized and underfit. We could parameterize and still overfit, with an acceptable change in accuracy.

The preliminary studies described in this report have demonstrated that data distribution shifts impact model prediction accuracy, specifically that the accuracy of a CNN, trained for a self-driving task under a certain data distribution regime, is expected to change if the data distribution changes, and that the change in accuracy is clearly noticed when the data distribution shift is positive, i.e. the individual pixel values increasing, the RGB image becoming brighter, and the distribution shifting to the right, and shown in Figure \ref{fig:RGBShiftsMinusAndPlus}.

Although these results are encouraging, two aspects of the work need to be addressed. The first is testing the hypotheses in a more realistic simulation scenario. The SDSandbox environment used in this report uses Unity as the game engine, and is subject to realistic simulations, however it does not represent actual urban layouts an autonomous vehicle would encounter, as well as other entities expected to be found in that setting such as alternative vehicle models, pedestrians, road layouts with intersections and other elements such as traffic lights and signs that determine and constrain driving, which the CARLA simulator should provide. The second aspect to be addressed is determining metrics to quantify data distributions shifts. This is in the author's view, the biggest gap in the research so far, as there are many options and a more thorough investigation on pros and cons is required to inform a decision.

Class imbalance is an issue that affects classifier networks. Regressor networks predict continuous values. Both classifier and regressor networks require training data. Data used for regressor networks may present some degree of skew if the expected continuous value is not uniformly distributed, which is always the case in the examples we studied. It remains then an open question is there could be a potential data imbalance issue with regressor network training data.
% I have had an article submission refused on grounds that 
% CANNOT FIND TRAIL - BAD

In the event that the approach proposed here is successful and adopted as a standard, there remains the question of how to associate a range of quantities that define the safe limits data supplied to the model. This would naturally present itself as metadata, which has long been the case for example, semiconductors, which are marketed to be used within pre-defined, current, voltage and temperature ranges, out of which the component cannot be guaranteed to operate as it would if within the recommended range \cite{horowitz1989art}.
% maybe The new Art of Electronics 





While is it generally acknowledge that predictive models must be "robust" i.e. invariant to data shifts, the initial findings shown here suggest that, for these specific cases i.e. given network architecture, training data, training regime and so forth, at a certain threshold of the data shift, the predictive accuracy of the network will rapidly degrade, that is, the average steering error presents a sharp rise. The model is not expected to be invariant to such shifts, as much as a human driver would not be. The case in point being a storm, where visibility is so compromised that it would be safer to park the vehicle and wait for the storm to blow over, or not start the journey at all, or a camera placed on an autonomous vehicle that experienced temporary obstruction or abrupt change in direction of view due to, for example, mechanical deformation due to a collision. In the scenario described, the issue is "safety", and not "robustness", where accuracy is not expected of the model in a case where a human would also be inaccurate. Further work is required around the usage of both terms.

Ultimately we want to produce metrics that would determine the safe operation of an autonomous system within the available data regime, such that data presented to system outside the know safe regime would require pausing and/or human intervention as shown in Figure \ref{fig:CARLA_Ticks}.
